ResFed: Communication Efficient Federated Learning by Transmitting Deep Compressed Residuals

Federated learning enables cooperative training among massively distributed clients by sharing their learned local model parameters. However, with increasing model size, deploying federated learning requires a large communication bandwidth, which limits its deployment in wireless networks. To address this bottleneck, we introduce a residual-based federated learning framework (ResFed), where residuals rather than model parameters are transmitted in communication networks for training. In particular, we integrate two pairs of shared predictors for the model prediction in both server-to-client and client-to-server communication. By employing a common prediction rule, both locally and globally updated models are always fully recoverable in clients and the server. We highlight that the residuals only indicate the quasi-update of a model in a single inter-round, and hence contain more dense information and have a lower entropy than the model, comparing to model weights and gradients. Based on this property, we further conduct lossy compression of the residuals by sparsification and quantization and encode them for efficient communication. The experimental evaluation shows that our ResFed needs remarkably less communication costs and achieves better accuracy by leveraging less sensitive residuals, compared to standard federated learning. For instance, to train a 4.08 MB CNN model on CIFAR-10 with 10 clients under non-independent and identically distributed (Non-IID) setting, our approach achieves a compression ratio over 700X in each communication round with minimum impact on the accuracy. To reach an accuracy of 70%, it saves around 99% of the total communication volume from 587.61 Mb to 6.79 Mb in up-streaming and to 4.61 Mb in down-streaming on average for all clients.

==> appendics/A_effectiveness.tex <==
Convergence




Assume the function is a Local Lipschitz continuity of the function $f$
\begin{equation}
    ||\nabla f(\hat w) - \nabla f(w_i)|| \leq L||\hat w - w_i||
\end{equation}

Based on the L-Lipschitz smoothness of f and Taylor expansion
\begin{equation}
    f(w_i) = f(\hat w + (w_i -\hat w)) \leq f(\hat w) + \nabla f(\hat w)^T(w_i -\hat w)+\frac{1}{2}L||w_i - \hat w||^2_2
\end{equation}

\begin{equation}
    \leq f(\hat w) - (1 - \frac{1}{2}L\eta)\eta||\nabla f(\hat w)||^2_2
\end{equation}

\begin{equation}
    f(w_i^t)-f(w_i^*)\leq \frac{||w_i^t-w_i^*||^2_2}{2\eta t} 
\end{equation}


\begin{equation}
    r_i^{t+1} \leq (\frac{t-1}{4\eta t(t+1) })||w_i^t-w_i^*||^2_2 \leq w_i^{t+1}
\end{equation}

==> appendics/algorithm_sim.tex <==

\begin{algorithm}[h]%Consider splitting the algo into server and client parts or use another template.
 \Reviewb{
 \caption{\raggedright: \Reviewb{Simplified residual-based federated learning framework}}
 \label{alg:FedRes}
 \begin{algorithmic}[1]

    \State \textbf{Server runs:} 
    \State initialize the global model, empty local and global model trajectories, and the predictor at the server
    \For{$i \in \{1,2,...,N\}$}
       \State initialize empty local and global model trajectories, and the predictor
       \State share the predictors
    \EndFor
    \For{each communication round}
        \For{each client \textbf{in parallel}}
            \If{$t < T$}
                \State do normal federated learning and update trajectories
            \Else
            \State \Reviewa{server communicates $\bar r_{i,dl}$ to the client $i$}
            \State $\bar r_{i,ul} \leftarrow$
            \textbf{ResFedClientUpdate} $(i, \bar r_{i,dl})$ \Comment{@client $i$}
            \State \Reviewa{client $i$ communicates $\bar r_{i,ul}$ to the server}
            \State recovery models $\hat w_i$ based on predicted models $\tilde w_i$
            \EndIf
         \State update local trajectory at the server
        \EndFor
        \State $w \leftarrow \textbf{Aggregate}(\hat w_1,...,\hat w_N)$
        \For {each client}
            \State compute residuals $r_{i,dl}$ based on predicted model $\tilde w_i$
            \State compress residuals $\bar r_{i,dl}$ and synchronize global trajectory
        \EndFor
    \EndFor
    \State \textbf{return} $w$ 
    \vspace{0.2cm}
    \State \textbf{ResFedClientUpdate} $(k, \bar r)$
    \State recover models $\hat w$ based on predicted models
    \State update global trajectory
    \State $w_k \leftarrow \textbf{LocalTrain}(\hat w)$
    \State compute residuals $r_k$ based on predicted models $\tilde w$
    \State compress residuals $\bar r_k$ and synchronize global trajectory
    \State \textbf{return} $\bar r_k$

\end{algorithmic}}
\end{algorithm}


==> appendics/extended_discussion.tex <==
\section{Extended Discussion}

In Sec.\ref{sec:warmup}, we discuss the potential enhancement from warn-up communication rounds, which has been employed in the previous work~\cite{lin2018deep} to increase the compression ratio for deep gradient compression.\Rui{tbd.}

Additionally, we provide primary evaluation on security improvement from \myResFed in Fig.~\ref{}\Rui{tbd.}, which is discussed in Sec.~\ref{sec:security}.




==> others/04_analysis.tex <==
\section{Analysis}
\label{sec:analysis}

\subsection{Residual Entropy}

\subsection{Model Prediction Accuracy}

\mypara{Non-IID}

\mypara{learning rate}

\mypara{local epochs}


\subsection{Lossy Compression}

(Entropy encoding has not been considered yet.)
Compression Ratio:
\begin{equation}
    \label{Eq:}
    CR = \frac{N*32}{(N-M)*2^L+M+2*L*32}
\end{equation}
where $N$ is the number of original residual parameters, which should be equal to the number of model parameters. We consider each parameter is a 32-bits float type and occupies 32-bits for serializing. $M$ is the number of pruned residual parameters. $L$ is the gridsearch for residual quantization.

Compression ratio changing

Accuracy vs compression ratio

Time to convergence vs round to convergence

Non-IID to compression






==> others/04_experiement.tex <==
\section{Experiment}
\label{sec:experiment}

\subsection{Experimental Settings}
Guided by the previous work by~\cite{caldas2018leaf}\cite{Li2020Fair}, we process and distribute the datasets MNIST~\cite{deng2012mnist}, CIFAR-10~\cite{Krizhevsky09learningmultiple}, CIFAR-100~\cite{Krizhevsky09learningmultiple} Tiny-ImageNet~\cite{tinyimagenet} on several clients, and train LeNet, 3-layer-CNN, ResNet-18 on those federated dataset distributively, as shown in Tab.~\ref{table:exp_settings}.  We provide more detailed information about the federated datasets in Appendix~\ref{sec:app_a}.
\input{others/tab_dataset}

%Communication volume for each round could be...
%The frequency can be set up to xx in In 5G NR environment
%The final time for convergence could be reduced by xx from xx to xx

%1. weight sampling
%2. residual sampling
%3. weight sampling after a while.





\subsection{Performance Comparison}

\mypara{Comparison with STC}
\cite{sattler2019robust}

\setlength{\tabcolsep}{3pt}
\begin{table*}[h]
\centering
\begin{threeparttable}
\caption{Comparison with STC for training a VGG11* on CIFAR10 distributed with 5 clients}
\label{table:comparison}

\begin{tabular}{C{4cm}|C{1.3cm}C{1.3cm}|C{1.3cm}C{1.3cm}}
\toprule %%%%%%%%%%%%%%%%%%


{Sparsity} & \multicolumn{2}{c|}{0.04} & \multicolumn{2}{c|}{0.0025}\\
\midrule %%%%%%%%%%%%%%%%%%
{Framework} & {STC} & {ResFed} & {STC} & {ResFed}\\
\midrule %%%%%%%%%%%%%%%%%%
{Acc. = 0.84} & {118.43 MB/1184.3 MB} & {ResFed} & {183.9 MB /1839 MB} & {ResFed}\\


{Sparsity} & \multicolumn{2}{c|}{VGG11*@CIFAR}\\
\midrule %%%%%%%%%%%%%%%%%%
{Framework} & {STC} & {ResFed} & {STC} & {ResFed}\\
\midrule %%%%%%%%%%%%%%%%%%
{Acc. = 0.84} & {118.43 MB/1184.3 MB} & {ResFed} & {183.9 MB /1839 MB} & {ResFed}\\

\bottomrule %%%%%%%%%%%%%%%%%%
\end{tabular}
\begin{tablenotes}
     \small
     \item[1]: STC:~\cite{sattler2019robust} Bidirectional

   \end{tablenotes}
\end{threeparttable}
\end{table*}

\mypara{Comparison with TC}
\cite{xu2020ternary}

\mypara{Comparison with FedZip}
\cite{}

\input{others/tab_comparison}

\subsection{Ablation Study}

\subsection{Influence of Hyperparameters}




==> others/algo1.tex <==

\begin{algorithm}[t]%Consider splitting the algo into server and client parts or use another template.
 \caption{\raggedright: \myResFed: Residual-based federated learning framework}
 \label{alg:FedRes}
 \begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Server Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \newcommand{\algorithmicbreak}{\textbf{break}}
 \newcommand{\BREAK}{\STATE \algorithmicbreak}
 \REQUIRE {predictor $h_{predictor}$ and compressor $h_{compressor}$}
 \renewcommand{\algorithmicrequire}{\textbf{Client Input:}}
 \REQUIRE {number of the client $N$, predictors $\{f_{predictor,i}|i = 1,2,...,N\}$, compressors $\{f_{compressor,i}|i = 1,2,...,N\}$}
 \ENSURE  {$\tilde w$}
    \\\STATE initialize the global model $w$ 
    \\\STATE initialize the empty model trajectories $\mathcal{T}, \mathcal{\hat T}_{1},...,\mathcal{\hat T}_{N}$
    \\\STATE initialize the predictor $h_{predictor}$
    %\\\textit{Sharing predictors}
    \\\FOR{$i \in \{1,2,...,N\}$}
        \STATE $h'_{predictor,i}=h_{predictor}$ 
        \STATE initialize the predictor $f_{predictor, i}$
        \STATE $f'_{predictor,i} = f_{predictor, i}$
    \ENDFOR
    \\\FOR{$t \in \{1,2,...\}$}
        %\textit {{Model prediction}}
        \STATE $\tilde w \leftarrow f_{predictor, i}(\mathcal{\hat T}_1,\mathcal{\hat T}_2,... \mathcal{T}, w)$
        %\textit{Computing Model Residuals}
        \STATE $r \leftarrow  w - \tilde w$
        %\textit{Compress Model Residuals}
        \STATE $\bar r \leftarrow h_{compression}(r)$
        %\textit{Trajectory Synchronization}
        \STATE $\hat w \leftarrow \tilde w + \bar r$
        \STATE $\mathcal{T} \leftarrow cache(\hat w)$
        \FOR{$i \in \{1,2,...,N\}$ \textbf{in parallel}}
            \STATE $\bar r_i \leftarrow$ \textbf{ResFedClientUpdate} $(i, \bar r)$
            \STATE $\hat w_i \leftarrow \tilde w_i + \bar r_i$
            \STATE $\mathcal{\hat T}_i \leftarrow cache(\hat w_i)$
            \STATE $\hat w_i \leftarrow \tilde w_i + \bar r_i$
        \ENDFOR
        \STATE $w \leftarrow aggregate(\hat w_i)$
    \ENDFOR
\end{algorithmic}
\end{algorithm}

==> others/algo1_simplified.tex <==

\begin{algorithm}[t]%Consider splitting the algo into server and client parts or use another template.
 \caption{\raggedright: \myResFed: Residual-based federated learning framework}
 \label{alg:FedRes_sim}
 \begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Server Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \newcommand{\algorithmicbreak}{\textbf{break}}
 \newcommand{\BREAK}{\STATE \algorithmicbreak}
 \REQUIRE {predictor $h_{predictor}$ and compressor $h_{compressor}$}
 \renewcommand{\algorithmicrequire}{\textbf{Client Input:}}
 \REQUIRE {number of the client $N$, predictors $\{f_{predictor,i}|i = 1,2,...,N\}$, compressors $\{f_{compressor,i}|i = 1,2,...,N\}$}
 \ENSURE  {$\tilde w$}
    \\\STATE initialize the global model $w$ 
    \\\STATE initialize the empty model trajectories $\mathcal{T}, \mathcal{\hat T}_{1},...,\mathcal{\hat T}_{N}$
    \\\STATE initialize the predictor $h_{predictor}$
    %\\\textit{Sharing predictors}
    \\\FOR{$i \in \{1,2,...,N\}$}
        \STATE $h'_{predictor,i}=h_{predictor}$ 
        \STATE initialize the predictor $f_{predictor, i}$
        \STATE $f'_{predictor,i} = f_{predictor, i}$
    \ENDFOR
    \\\FOR{$t \in \{1,2,...\}$}
        %\textit {{Model prediction}}
        \STATE $\tilde w \leftarrow f_{predictor, i}(\mathcal{\hat T}_1,\mathcal{\hat T}_2,... \mathcal{T}, w)$
        %\textit{Computing Model Residuals}
        \STATE $r \leftarrow  w - \tilde w$
        %\textit{Compress Model Residuals}
        \STATE $\bar r \leftarrow h_{compression}(r)$
        %\textit{Trajectory Synchronization}
        \STATE $\hat w \leftarrow \tilde w + \bar r$
        \STATE $\mathcal{T} \leftarrow cache(\hat w)$
        \FOR{$i \in \{1,2,...,N\}$ \textbf{in parallel}}
            \STATE $\bar r_i \leftarrow$ \textbf{ResFedClientUpdate} $(i, \bar r)$
            \STATE $\hat w_i \leftarrow \tilde w_i + \bar r_i$
            \STATE $\mathcal{\hat T}_i \leftarrow cache(\hat w_i)$
            \STATE $\hat w_i \leftarrow \tilde w_i + \bar r_i$
        \ENDFOR
        \STATE $w \leftarrow aggregate(\hat w_i)$
    \ENDFOR
\end{algorithmic}
\end{algorithm}

==> others/tab_comparison.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table*}[!ht]
\centering
\fontsize{8}{12}\selectfont
%\bgroup\footnotesize
\begin{threeparttable}
\caption{Comparison.}
\label{table:comparison}

\begin{tabular}{C{4cm}|C{1.3cm}C{1.3cm}|C{1.3cm}C{1.3cm}|C{1.3cm}C{1.3cm}}
\toprule %%%%%%%%%%%%%%%%%%

{Framework} & \multicolumn{2}{c|}{Parameter bits} & \multicolumn{2}{c|}{Compression ratio}  & \multicolumn{2}{c}{Testing Error} \\
{Framework} & {Upload} & {Download} & {Upload} & {Download} & {Top 1\%} & {Top 10\%} \\

\midrule %%%%%%%%%%%%%%%%%%

{Baseline (FedAvg)} & {} & {} & {} & {} & {} & {}\\
{STC~\cite{sattler2019robust}}  & {} & {} & {} & {} & {} & {}\\
{FTTQ~\cite{xu2020ternary}}  & {} & {} & {} & {} & {} & {}\\
{FedPAQ~\cite{reisizadeh2020fedpaq}} & {} & {} & {} & {} & {} & {}\\
{UVeQFed~\cite{shlezinger2020uveqfed}}  & {} & {} & {} & {} & {} & {}\\
{FedZIP~\cite{malekijoo2021fedzip}}  & {} & {} & {} & {} & {} & {}\\
{DAdaQuant~\cite{honig2022dadaquant}}  & {} & {} & {} & {} & {} & {} \\
{ResFed}  & {} & {} & {} & {} & {} & {}\\

\bottomrule %%%%%%%%%%%%%%%%%%
\end{tabular}
\begin{tablenotes}
     \small
     \item[1]: STC:~\cite{sattler2019robust} Bidirectional
     \item[2]: FTTQ:~\cite{xu2020ternary} uploading
     \item[3]: FedPAQ:~\cite{reisizadeh2020fedpaq} uploading 
     \item[4]: FedZIP:~\cite{malekijoo2021fedzip} Bidirectional
     \item[5]: DAdaQuant:~\cite{honig2022dadaquant} uploading
   \end{tablenotes}
\end{threeparttable}
\end{table*}





==> sections/06_discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\subsection{A Few Warm-up Communication Rounds}
\label{sec:warmup}

\subsection{Further benefits by communicating residuals}

\mypara{Security}
\label{sec:security}
% Add some miss labels in one client

\mypara{Privacy}
% ??

\mypara{Robustness}
%Add some error in updating for one client?

\subsection{limitations}
\label{sec:limitations}
We cache the recovered models as local and global trajectories for continual model prediction and residual computing in all clients and server. Assuming that we perform \myResFed with $N$ clients for training a model with $V$ 32-bit float parameters and we set the trajectory length on $T$. Then each client should use $2*32*V*T$ bits memory to cache the $2$ trajectories. Thus, the additional required memory size in each client is linear increased with $T$ and $V$. For the server, it needs $2*32*V*T*N$ bits memory to cache the local and global trajectories for all clients. 

==> sections/09_ethics_statement.tex <==
\section{Ethics statement}
\Rui{Do we need this?}
